UAV attitude estimation using Unscented Kalman Filter and TRIAD

A main problem in autonomous vehicles in general, and in \acp{UAV} in particular, is the determination of the attitude angles. A novel method to estimate these angles using off-the-shelf components is presented. This paper introduces an \ac{AHRS} based on the \ac{UKF} using the \ac{TRIAD} algorithm as the observation model. The performance of the method is assessed through simulations and compared to an \ac{AHRS} based on the \ac{EKF}. The paper presents field experiment results using a real fixed-wing \ac{UAV}. The results show good real-time performance with low computational cost in a microcontroller.

==> Makefile <==
SOURCES := \
		  modif.tex
EPS_IMAGES := $(wildcard images/*.eps)
IMAGES := $(EPS_IMAGES) $(wildcard images/*.jpg images/*.png)

texlive_V := $(shell sh -c "pdflatex --version | sed -n -e '1s-^.*TeX Live \([0-9]\{4\}\).*-\1-p'")

ifeq ($(texlive_V),2009)
	EPS_IMAGES_TO_BUILD := $(EPS_IMAGES)
else
	EPS_IMAGES_TO_BUILD :=
endif

.PHONY: clean all-clean build-images

all: modif.pdf

build-images: $(EPS_IMAGES_TO_BUILD)
	[ -n "$(EPS_IMAGES_TO_BUILD)" ] && for i in $(EPS_IMAGES_TO_BUILD) ; do epstopdf $$i ; done || true

clean:
	$(RM) *~ *.pdf *.dvi *.log *.aux *.bbl *.blg *.toc *.lol *.loa *.lox \
		*.lot *.out *.lg *.tmp *.xref

all-clean: clean
	$(RM) *-converted-to.pdf $(patsubst %.eps,%.pdf,$(EPS_IMAGES))

modif.pdf: modif.tex $(IMAGES) build-images
	pdflatex modif
	bibtex modif
	pdflatex modif
	pdflatex modif

modif: modif.tex $(IMAGES)
	pdflatex modif
	bibtex modif
	pdflatex modif
	pdflatex modif

